Best Practices for 2-Body Pose Forecasting

The task of collaborative human pose forecasting stands for predicting the future poses of multiple interacting people, given those in previous frames. Predicting two people in interaction, instead of each separately, promises better performance, due to their body-body motion correlations. But the task has remained so far primarily unexplored. In this paper, we review the progress in human pose forecasting and provide an in-depth assessment of the single-person practices that perform best for 2-body collaborative motion forecasting. Our study confirms the positive impact of frequency input representations, space-time separable and fully-learnable interaction adjacencies for the encoding GCN and FC decoding. Other single-person practices do not transfer to 2-body, so the proposed best ones do not include hierarchical body modeling or attention-based interaction encoding. We further contribute a novel initialization procedure for the 2-body spatial interaction parameters of the encoder, which benefits performance and stability. Altogether, our proposed 2-body pose forecasting best practices yield a performance improvement of 21.9% over the state-of-the-art on the most recent ExPI dataset, whereby the novel initialization accounts for 3.5%. See our project page at https://www.pinlab.org/bestpractices2body

==> Tables/actions_description.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{cc}
Action & Name \\ \hline
$A_1$   & A-frame     \\
$A_2$   & Around the back     \\
$A_3$   &  Coochie    \\
$A_4$   &  Frog classic    \\
$A_5$   &   Noser   \\
$A_6$   &   Toss out   \\
$A_7$   &    Cartwheel  \\ \hline
$A_8$   &    Back flip  \\
$A_9$   &    Big ben  \\
$A_{10}$   &    Chandelle  \\
$A_{11}$   &   Check the challenge   \\
$A_{12}$   &    Frog-turn  \\
$A_{13}$   &     Twisted toss \\ \hline
$A_{14}$   &   Crunch-toast   \\
$A_{15}$   &    Frog-kick  \\
$A_{16}$   &   Ninja-kick  
\end{tabular}
\caption{List of actions and their corresponding names}
\label{tab:actions}
\end{table}

==> Tables/expit_ame.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}

% \begin{table*}[!ht]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c}
% \hline
%  \multicolumn{1}{c|}{\textit{Action}}                      & \multicolumn{4}{c|}{A1 A-frame}                                                    & \multicolumn{4}{c|}{A2 Around the back}                                            & \multicolumn{4}{c|}{A3 Coochie}                                                                  & \multicolumn{4}{c|}{A4 Frog classic}                                               & \multicolumn{4}{c|}{A5 Noser}                                                      & \multicolumn{4}{c|}{A6 Toss Out}                                                   & \multicolumn{4}{c|}{A7 Cartwheel}                                                  & \multicolumn{4}{c}{Average $\downarrow$}                                                       \\ \hline
% \multicolumn{1}{c|}{\textit{Time (msec)}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}}               & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} \\ \hline \hline
% LTD~\cite{mao19ltd}                                          & 70                 & 125                & 157                & 189                 & 131                & 242                & 321                & 426                 & 102                & 194                & 260                & \multicolumn{1}{c|}{357}          & 62                 & 117                & 155                & 197                 & 72                 & 131                & 173                & 231                 & 81                 & 151                & 200                & 280                 & 112                & 223                & 315                & 442                 & 90                 & 169                & 226                & 303                 \\
%  HisRep~\cite{mao20his}                                           & 52                 & 103                & 139                & 188                 & 96                 & 186                & 256                & 349                 & 57                 & 118                & 167                & \multicolumn{1}{c|}{240}          & 45                 & 93                 & 131                & 180                 & 51                 & 105                & 149                & 214                 & 61                 & 125                & 176                & 252                 & 71                 & 150                & 222                & 333                 & 62                 & 126                & 177                & 251                 \\
%  MSR-GCN~\cite{Dang21}                                         & 56                 & 100                & 132                & 175                 & 102                & 187                & 256                & 365                 & 65                 & 120                & 166                & \multicolumn{1}{c|}{244}          & 50                 & 95                 & 127                & 172                 & 54                 & 100                & 138                & 202                 & 70                 & 132                & 182                & 258                 & 82                 & 154                & 218                & 321                 & 69                 & 127                & 174                & 248                 \\
% siMLPe~\cite{guo2022back}                                  & 49                 & 102                 & 137                & 177                 & 88                 & 180                & 244                & 336                 & 57                 & 122                & 174                & \multicolumn{1}{c|}{254}          & 45                 & 100                 & 137                & 182                 & 50                 & 103                 & 144                & 206                 & 59                 & 126                & 175                & 250                 & 77                 & 164                & 134                & 348                 & 60                 & 128                & 178                & 250                 \\ 
% XIA~\cite{guo21}                                  & 49                 & 98                 & 140                & 192                 & 84                 & 166                & 234                & 346                 & 51                 & 105                & 154                & \multicolumn{1}{c|}{234}          & 41                 & 84                 & 120                & 161                 & 43                 & 90                 & 132                & 197                 & 55                 & 113                & 163                & 242                 & 62                 & 130                & 192                & 291                 & 55                 & 112                & 162                & 238                 \\ 

% Ours                               & \textbf{34}        & \textbf{71}        & \textbf{105}       & \textbf{159}        & \textbf{56}        & \textbf{121}       & \textbf{181}       & \textbf{292}        & \textbf{36}        & \textbf{78}        & \textbf{118}       & \multicolumn{1}{c|}{\textbf{195}} & \textbf{30}        & \textbf{66}        & \textbf{98}       & \textbf{145}        & \textbf{35}        & \textbf{74}        & \textbf{113}       & \textbf{171}        & \textbf{41}        & \textbf{88}        & \textbf{129}       & \textbf{193}        & \textbf{47}        & \textbf{108}       & \textbf{166}       & \textbf{261}        & \textbf{39}        & \textbf{86}        & \textbf{129}       & \textbf{202}        \\ \hline 

% \end{tabular}}
% \caption{Results in millimeters for ExPI Common actions split. Our model achieves state-of-the-art results in all actions considered, at each predicted time instant.\LS{Are the fonts in the table too small? Will this be an infringement of the guidelines?} }
% \label{tab:expi}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[!ht]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c|c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c@{\hspace{0.3\tabcolsep}}c}
\hline
 \multicolumn{1}{c|}{\textit{Action}}                      & \multicolumn{4}{c|}{A1}                                                    & \multicolumn{4}{c|}{A2}                                            & \multicolumn{4}{c|}{A3}                                                                  & \multicolumn{4}{c|}{A4}                                               & \multicolumn{4}{c|}{A5}                                                      & \multicolumn{4}{c|}{A6}                                                   & \multicolumn{4}{c|}{A7}                                                  & \multicolumn{4}{c}{Average $\downarrow$}                                                       \\ \hline
\multicolumn{1}{c|}{\textit{Time (msec)}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}}               & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} \\ \hline \hline
LTD~\cite{mao19ltd}                                           & 51                 & 92                 & 116                & 132                 & 51                 & 91                 & 116                & 148                 & 43                 & 80                 & 103                & \multicolumn{1}{c|}{130}          & 38                 & 70                 & 89                 & 111                 & 39                 & 70                 & 90                 & 116                 & 42                 & 75                 & 94                 & 123                 & 52                 & 101                & 139                & 198                 & 45                 & 83                 & 107                & 137                 \\
 HisRep~\cite{mao20his}                                    & 34                 & 69                 & 97                 & 130                 & 44                 & 84                 & 115                & 150                 & 32                 & 65                 & 91                 & \multicolumn{1}{c|}{121}          & 27                 & 56                 & 82                 & 112                 & 28                 & 58                 & 85                 & 121                 & 34                 & 66                 & 88                 & 115                 & 42                 & 83                 & 120                & 171                 & 34                 & 69                 & 97                 & 131                 \\
 MSR-GCN~\cite{Dang21}                                   & 41                 & 75                 & 99                 & 126                 & 54                 & 96                 & 129                & 180                 & 41                 & 74                 & 98                 & \multicolumn{1}{c|}{135}          & 34                 & 61                 & 82                 & 106                 & 33                 & 59                 & 79                 & 109                 & 42                 & 71                 & 93                 & 124                 & 57                 & 103                & 146                & 210                 & 43                 & 77                 & 104                & 141                 \\
MRT~\cite{wang21}                                &  34 & 69 & 95 & 128 & 39 & 78 & 106 & 142 & 30 & 59 & 83 & 115 & 28 & 57 & 79 & 110 & 28 & 57 & 79 & 108 & 34 & 68 & 91 & 120 & 39 & 80 & 114 & 160 & 33 & 67 & 92 & 126                 \\ 
siMLPe~\cite{guo2022back}                                &  32 & 69 & 94 & 115 & 44 & 93 & 122 & 160 & 33 & 73 & 102 & 138 & 26 & 61 & 87 & 114 & 28 & 60 & 84 & 112 & 32 & 69 & 93 & 123 & 45 & 94 & 127 & 171 & 34 & 74 & 101 & 133                 \\ 
XIA~\cite{guo21}                                 & 32                 & 68                 & 99                 & 128                 & 41                 & 82                 & 116                & 163                 & 29                 & 58                 & 84                 & \multicolumn{1}{c|}{116}          & 24        & 50                 & 73                 & 96                  & 24        & 51        & 75                 & 109                 & 31        & 62                 & 86                 & 114                 & 41                 & 81                 & 115                & 160                 & 32                 & 65                 & 93                 & 127                 \\

Ours                         &   \textbf{24} & \textbf{51} & \textbf{76} & \textbf{114} & \textbf{31} & \textbf{66} & \textbf{93} & \textbf{132} & \textbf{23} & \textbf{49} & \textbf{70} & \textbf{103} & \textbf{19} & \textbf{41} & \textbf{60} & \textbf{85} & \textbf{21} & \textbf{44} & \textbf{64} & \textbf{93} & \textbf{24} & \textbf{52} & \textbf{73} & \textbf{100} & \textbf{29} & \textbf{64} & \textbf{95} & \textbf{143} & \textbf{24} & \textbf{52} & \textbf{76} & \textbf{110}        \\ \hline 

\end{tabular}}
\caption{Results in millimeters for ExPI Common actions split. Our model achieves state-of-the-art results in all actions considered, at each predicted time instant.}
\label{tab:expi_ame}
\end{table*}

==> Tables/init.tex <==
% \begin{table}[!htb]
% \centering
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{lcccc}
% \hline
%                                           & \multicolumn{4}{c}{JME (std) $\downarrow$}                                                       \\ \cline{2-5}
% \multicolumn{1}{l}{\textit{Time Horizon (msec)}} & {\textit{160}} & {\textit{400}} & {\textit{560}} & {\textit{1000}} \\ \hline \hline
% \multicolumn{1}{l|}{Uniform}               & 40.5               & 89.0               & 133.9               & 207.6               \\
% \multicolumn{1}{l|}{Glorot et al.\cite{glorot10}}                 & 40.3 (0.1)               & 89.4 (1.2)               & 134.3 (1.5)               & 207.9 (1.8)              \\
% \multicolumn{1}{l|}{He et al.\cite{he15}}                 & 40.2 (0.4)               & 88.6 (0.7)               & 133.4 (1.4)               & 206.6 (1.2)               \\
% \multicolumn{1}{l|}{Ours}                 & \textbf{39.7} (0.4)               & \textbf{87.6} (1.0)               & 131.8 (1.7)               & 205.1 (1.4)             \\
% \multicolumn{1}{l|}{Ours w/ inductive bias}                 & 40.0 \textbf{(0.05)}             & \textbf{87.6 ($\pm$0.1)}              & \textbf{131.6 (0.2)}                & \textbf{205.0 (0.9)}               \\

% \end{tabular}}
% \caption{Initialization procedures.}
% \label{tab:init}
% \end{table}


\begin{table}[!htb]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc}
\hline
                                          & \multicolumn{4}{c}{JME (std) $\downarrow$}                                                       \\ \cline{2-5}
\multicolumn{1}{l}{\textit{Time Horizon (msec)}} & {\textit{160}} & {\textit{400}} & {\textit{560}} & {\textit{1000}} \\ \hline \hline
\multicolumn{1}{l|}{Uniform}               & 39.7 ($\pm$0.7)              & 87,6 ($\pm$0.7)              & 132.2 ($\pm$0.5)              & 207.7 ($\pm$1.0)              \\
\multicolumn{1}{l|}{Glorot et al.\cite{glorot10}}                 & 40.3 ($\pm$0.1)               & 89.4 ($\pm$1.2)               & 134.3 ($\pm$1.5)               & 207.9 ($\pm$1.8)              \\
\multicolumn{1}{l|}{He et al.\cite{he15}}                 & 40.2 ($\pm$0.4)               & 88.6 ($\pm$0.7)               & 133.4 ($\pm$1.4)               & 206.6 ($\pm$1.2)               \\
\multicolumn{1}{l|}{Ours}                 & \textbf{39.7} ($\pm$0.4)               & \textbf{87.6} ($\pm$1.0)               & 131.8 ($\pm$1.7)               & 205.1 ($\pm$1.4)             \\
\multicolumn{1}{l|}{Ours w/ inductive bias}                 & 40.0 \textbf{($\pm$0.05)}             & \textbf{87.6 ($\pm$0.1)}              & \textbf{131.6 ($\pm$0.2)}                & \textbf{205.0 ($\pm$0.9)}               \\ \hline

\end{tabular}}
\caption{Initialization procedures. \FG{Improvements are small. One should clarify that we refer here to the best possible model, already. May we add the results of init also on the base model, where they should be larger? If it stays so, the inductive bias part should be removed. But there is already a nice story in the paper, so improving the inductive is not a priority. Our priority is the paper and a good story into the ablations.}}
\label{tab:init}
\end{table}

==> Tables/iterative.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!h]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ccccccc}
\hline
                                               &                       &                        & \multicolumn{4}{c}{MPJPE (ms)$\downarrow$}                                                           \\ \cline{4-7} 
\multicolumn{1}{c}{}                          & \textit{Input Frames} & \textit{Output Frames} & {  \textit{200}} & {  \textit{400}} & {  \textit{600}} & {  \textit{1000}} \\ \hline \hline
 & 50                    & 1                      & 43                 & 113                & 176                & 274                 \\
\multicolumn{1}{c}{}                         & 50                    & 5                      & 52                 & 114                & 162                & 243                 \\
\multicolumn{1}{c}{}                         & 50                    & 10                     & 62                 & 126                & 174                & 243                 \\
\multicolumn{1}{c}{}                         & 50                    & 50                     & 68                 & 131                & 177                & 244                 \\ \cline{2-7} 


\multicolumn{1}{c}{}                         & 10                    & 1                      & \textbf{36}               &   98                 &  164                  &  294                   \\
\multicolumn{1}{c}{}                         & 10                    & 5                      & 37                 & 89               & 141                & 238                 \\ 
 \textit{Used} & 10                    & 10                     & 39 & \textbf{86} & \textbf{129} & \textbf{202}       \\ \hline


\end{tabular}}
\caption{Results in millimeters on the ExPI dataset, on average common actions split. 
We show the impact that different combinations of input-output frames have on performance. 
Using 10 input frames makes predictions in the short term more accurate, helping results to be more stable in the long term.}
\label{tab:iterative}
\end{table}

==> Tables/single_ame.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[!htb]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c}
% \hline
% \multicolumn{1}{c|}{\textit{Action}}             & \multicolumn{4}{c|}{A1 A-frame}                         & \multicolumn{4}{c|}{A2 Around the back}                  & \multicolumn{4}{c|}{A3 Coochie}                          & \multicolumn{4}{c|}{A4 Frog classic}                    & \multicolumn{4}{c|}{A5 Noser}                           & \multicolumn{4}{c|}{A6 Toss Out}                         & \multicolumn{4}{c}{A7 Cartwheel}                        \\ \hline  
% \multicolumn{1}{c|}{\textit{Time (msec)}} & \textit{200}         & \textit{400}         & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}          & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}          & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}         & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}         & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}          & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}          & \textit{600}          & \textit{1000}         \\ \hline \hline
% LTD~\cite{mao19ltd}                                     & 70          & 126         & 155          & 183          & 131         & 243          & 312          & 415          & 102         & 194          & 252          & 338          & 62          & 117         & 153          & 203          & 71          & 131         & 171          & 231          & 81          & 151          & 199          & 299          & 112         & 223          & 306          & 411          \\
% HisRep~\cite{mao20his}                                  & 66          & 118         & 153          & 190          & 128         & 231          & 308          & 417          & 74          & 143          & 205          & 295          & 64          & 120         & 159          & 191          & 63          & 121         & 166          & 227          & 90          & 168          & 232          & 312          & 88          & 166          & 232          & 332          \\
% MSR-GCN~\cite{Dang21}                                 & 64          & 108         & 136          & \textbf{170}          & 119         & 210          & 282          & 385          & 79          & 144          & 189          & 265          & 59          & 103         & 134          & 173          & 65          & 118         & 162          & 225          & 86          & 151          & 201          & 283          & 96          & 178          & 255          & 362          \\
% siMLPe~\cite{guo2022back}                         & 60          & 113         & 145          & 200          & 104         & 202          & 268          & 373          & 76 & 150 & 205 & 305          & 58          & 110         & 151          & 203          & 64          & 123         & 163          & 218          & 76          & 152          & 207          & 277          & 93 & 180 & 254 & 341 \\ 
% XIA~\cite{guo21}                         & 64          & 120         & 160          & 199          & 109         & 200          & 275          & 381          & 59 & 117 & 174 & 277          & 60          & 116         & 162          & 209          & 53          & 106         & 152          & 221          & 65          & 122          & 166          & 223          & 74 & 144 & \textbf{203} & \textbf{301} \\ 

% Ours                            & \textbf{52} & \textbf{94} & \textbf{128} & 179 & \textbf{89} & \textbf{176} & \textbf{242} & \textbf{329} & \textbf{42}          & \textbf{90}          & \textbf{129}          & \textbf{200} & \textbf{49} & \textbf{96} & \textbf{134} & \textbf{185} & \textbf{48} & \textbf{99} & \textbf{140} & \textbf{196} & \textbf{52} & \textbf{105} & \textbf{144} & \textbf{198} & \textbf{68} & \textbf{140}          & 204         & 305          \\ \hline
% \end{tabular}}
% \caption{Results in millimeters for ExPI Single actions split. We outperform in 6 out of 7 stocks all baselines considered according to the MPJPE metric. For the other stocks our model is comparable with the current state of the art.}
% \label{tab:single}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!htb]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c}
\hline
\multicolumn{1}{c|}{\textit{Action}}             & \multicolumn{4}{c|}{A1}                         & \multicolumn{4}{c|}{A2}                  & \multicolumn{4}{c|}{A3}                          & \multicolumn{4}{c|}{A4}                    & \multicolumn{4}{c|}{A5}                           & \multicolumn{4}{c|}{A6}                         & \multicolumn{4}{c}{A7}                        \\ \hline  
\multicolumn{1}{c|}{\textit{Time (msec)}} & \textit{200}         & \textit{400}         & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}          & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}          & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}         & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}         & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}          & \textit{600}          & \textit{1000}         & \textit{200}         & \textit{400}          & \textit{600}          & \textit{1000}         \\ \hline \hline
LTD~\cite{mao19ltd}                                      & 51          & 99          & 129          & 163          & 61          & 110          & 150          & 229          & 53          & 96           & 131          & 188          & 46          & 81          & 106          & 142          & 44          & 79          & 106          & 147          & 53          & 100          & 162          & 176          & 70          & 133          & 163          & 198          \\
HisRep~\cite{mao20his}                                  & 51          & 93          & 114          & 127          & 51          & 91           & 116          & 162          & 43          & 80           & 100          & 126          & 38          & 70          & 88           & 118          & 39          & 70          & 90           & 125          & 42          & 75           & 93           & 123          & 52          & 101          & 137          & 188          \\
MSR-GCN~\cite{Dang21}                                 & 45          & 83          & 106          & 118          & 57          & 102          & 135          & 178          & 39          & 72           & 100          & 132          & 41          & 77          & 103          & 119          & 35          & 70          & 97           & 125          & 46          & 82           & 107          & 137          & 48          & 90           & 121          & 169          \\
MRT~\cite{wang21}                     &    36 & 69 & 93 & 123 & 44 & 81 & 106 & 138 & 41 & 76 & 96 & 114 & 30 & 61 & 81 & 105 & 33 & 64 & 88 & 121 & 34 & 64 & 83 & 104 & 42 & 83 & 114 & 157  \\
siMLPe~\cite{guo2022back}                     &    43 & 84 & 107 & 137 & 55 & 107 & 142 & 182 & 47 & 91 & 120 & 164 & 39 & 76 & 101 & 129 & 38 & 75 & 99 & 128 & 47 & 90 & 118 & 150 & 58 & 110 & 150 & 197  \\ 
XIA~\cite{guo21}                         & 43          & 84          & 115          & 131          & 53          & 99           & 136          & 185          & 35 & 68  & 98  & 140          & 37          & 74          & 106          & 128          & 29 & 59          & 86           & 125          & 39          & 72           & 94           & 119          & 43 & 82  & 112 & \textbf{152} \\

Ours                   &         \textbf{34} & \textbf{63} & \textbf{86} & \textbf{115} & \textbf{41} & \textbf{79} & \textbf{105} & \textbf{138} & \textbf{27} & \textbf{55} & \textbf{77} & \textbf{110} & \textbf{31} & \textbf{64} & \textbf{88} & \textbf{119} & \textbf{27} & \textbf{55} & \textbf{77} & \textbf{107} & \textbf{30} & \textbf{58} & \textbf{78} & \textbf{103} & \textbf{38} & \textbf{78} & \textbf{109} & 154       \\ \hline
\end{tabular}}
\caption{Results in millimeters for ExPI Single actions split. We outperform in 6 out of 7 stocks all baselines considered according to the MPJPE metric. For the other stocks our model is comparable with the current state of the art.}
\label{tab:single_ame}
\end{table*}

==> Tables/tab_rebuttal.tex <==

\begin{table}[h]
% \rowcolors{3}{gray!12}{white}
\resizebox{.48\textwidth}{!}{
\begin{tabular}{ccccccc} 
\hline
\textbf{Model} & \multicolumn{2}{|c|}{\textbf{Best Practices}} &   \multicolumn{4}{c}{\textit{\textbf{MPJPE} $\downarrow$}} \\

 & \multicolumn{1}{|c}{Freq. Enc.} & \multicolumn{1}{c|}{FC} & \textit{200} &\textit{400} & \textit{600}	& \multicolumn{1}{c}{\textit{1000}} \\ \hline \hline
\multicolumn{1}{l}{\textit{Wang et al.}} &&             & 70           & 127               & 176          & 248               \\
\hline
[19] &  & & 55 & 112 & 162 & 253 \\
siMLPe [19] &  & \checkmark & 63 & 128 & 177 & 249 \\
siMLPe & \checkmark & & 50 & 120 & 175 & 257 \\
siMLPe & \checkmark & \checkmark & 60 & 128 & 178 & 250 \\
siMLPe10 &  &  & 38 & 89 & 144 & 247 \\
siMLPe10 & \checkmark &  & 39 & 91 & 143 & 238 \\
siMLPe10 &  & \checkmark & 45 & 109 & 162 & 242 \\
siMLPe10 & \checkmark & \checkmark & 32 & 84 & 135 & 221 \\

\hline
Ours &  & & 55 & 112 & 156 & 224 \\
Ours & & \checkmark & 51 & 104 & 145 & 212 \\
Ours & \checkmark & & 41 & 88 & 135 & 219 \\
Ours & \checkmark & \checkmark & \textbf{39} & \textbf{86} & \textbf{129} & \textbf{202} \\

\hline
\end{tabular}}
\caption{ Error in millimeters on ExPI Common actions split with some of the best practices \AF{@fabio we add different format to cite siMLPe, which one is better?}} \RA{simple10 is with 10 input frames at the input and doing iterative prediction and the results could make sense if we say which components are best (here Freq. Enc. and FC). But we cannot put them as it is very good on short term}
\FG{I imagine we leave here only wang et al and ours with all best practices. putting best practices is not needed, unless wanting to remark what best practices wang et al are using. Also, you might want to remark that your report "Ours (w/ best practices)"}
\label{tab:ablation}

\end{table}


==> Tables/unseen_ame.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[normalem]{ulem}
% % \useunder{  ine}{  }{}
% \begin{table*}[!htb]
% \centering
% % \addtolength{\tabcolsep}{-2pt}

% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|
% c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|
% c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|
% c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c}
% \hline
%  \multicolumn{1}{c|}{\textit{Action}}                     & \multicolumn{3}{c|}{A8 - Back flip}                     & \multicolumn{3}{c|}{A9 - Big ben}                     & \multicolumn{3}{c|}{A10 - Chandelle}                                      & \multicolumn{3}{c|}{A11 - Check change}                                      & \multicolumn{3}{c|}{A12 - Frog turn}                                      & \multicolumn{3}{c|}{A13 - Twisted toss}                                      & \multicolumn{3}{c|}{A14 - Crunch-toast}                                      & \multicolumn{3}{c|}{A15 - Frog-ick}                                      & \multicolumn{3}{c|}{A16 - Ninja-kick}                                      & \multicolumn{3}{c}{Average $\downarrow$}                                  \\ \hline 
%  \multicolumn{1}{c|}{\textit{Time (msec)}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} \\ \hline \hline
% LTD~\cite{mao19ltd}                                              & 252          & 333          & 387           & 174          & 228          & 268           & 139                & 184                & 217                 & 239                & 324                & 394                 & 175                & 226                & 259                 & 148                & 191                & 220                 & 176                & 240                & 286                 & 143                & 178                & 192                 & 146                & 193                & 226                 & 177                & 233                & 272                 \\
% HisRep~\cite{mao20his}                                           & 157          & 219          & 257           & 134          & 190          & 233           & 96                 & 146                & 187                 & 195                & 283                & 358                 & 121                & 169                & 206                 & 92                 & 129                & \textbf{160}                 & 129                & 193                & 245                 & 80                 & 104                & 121                 & 112                & 154                & 187                 & 124                & 176                & 218                 \\
% MSR-GCN~\cite{Dang21}                                          & 177          & 239          & 295           & 143          & 179          & 213           & 157                & 222                & 281                 & 230                & 289                & 335                 & 188                & 245                & 290                 & 148                & 198                & 248                 & 234                & 319                & 384                 & 176                & 232                & 278                 & 162                & 218                & 266                 & 179                & 238                & 288                 \\
% siMLPe~\cite{guo2022back}                                  & 165          & 220          & 258           & 137          & 198          & 246           & 104                 & 154                & 198                 & 210                & 301                & 432                 & 114      & 156       & 187        & 94        & 132       & 160       & 140       & 204       & 255        & 91        & 119       & 138        & 120                & 166                & 204                 & 131                & 183                & 225                 \\ 
% XIA~\cite{guo21}                                  & 156          & 216          & 256           & 126          & 175          & 213           & 96                 & 152                & 205                 & 191                & 287                & 377                 & 118      & 165       & 203        & 91        & 129       & 162       & 122       & 183       & 232        & 81        & \textbf{107}       & \textbf{128}        & 106                & 150                & 185                 & 121                & 174                & 218                 \\ 

% Ours                               & \textbf{113} & \textbf{164} & \textbf{203}  & \textbf{114}  & \textbf{167} & \textbf{209}  & \textbf{85}        & \textbf{136}       & \textbf{183}        & \textbf{153}       & \textbf{231}       & \textbf{304}        & \textbf{100}                & \textbf{148}                & \textbf{188}                & \textbf{82}                 & \textbf{125}                & 162                 & \textbf{91}                & \textbf{138}                & \textbf{179}                 & \textbf{79}                & 109               & 132                 & \textbf{85}        & \textbf{124}       & \textbf{156}        & \textbf{100}       & \textbf{149}       & \textbf{191}        \\ \hline
% \end{tabular}}
% \caption{Results in millimeters for ExPI Unseen actions split. On average, we outperform the baseline considered over short and long time horizons. } 
% \label{tab:unseen}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{  ine}{  }{}
\begin{table*}[!htb]
\centering
% \addtolength{\tabcolsep}{-2pt}

\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|
c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|
c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|
c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c|c@{\hspace{0.7\tabcolsep}}c@{\hspace{0.7\tabcolsep}}c}
\hline
 \multicolumn{1}{c|}{\textit{Action}}                     & \multicolumn{3}{c|}{A8}                     & \multicolumn{3}{c|}{A9}                     & \multicolumn{3}{c|}{A10}                                      & \multicolumn{3}{c|}{A11}                                      & \multicolumn{3}{c|}{A12}                                      & \multicolumn{3}{c|}{A13}                                      & \multicolumn{3}{c|}{A14}                                      & \multicolumn{3}{c|}{A15}                                      & \multicolumn{3}{c|}{A16}                                      & \multicolumn{3}{c}{Average $\downarrow$}                                  \\ \hline 
 \multicolumn{1}{c|}{\textit{Time (msec)}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} & {   \textit{400}} & {   \textit{600}} & {   \textit{800}} \\ \hline \hline
LTD~\cite{mao19ltd}                                              & 106          & 136          & 155           & 91           & 119          & 135           & 72                 & 96                 & 116                 & 95                 & 123                & 146                 & 85                 & 106                & 116                 & 74                 & 91                 & 101                 & 86                 & 115                & 137                 & 98                 & 125                & 134                 & 85                 & 110                & 124                 & 88                 & 113                & 129                 \\
HisRep~\cite{mao20his}                                           & 86           & 120          & 142           & 73           & 104          & 128           & 54                 & 82                 & 104                 & 101                & 144                & 476                 & 61                 & 82                 & 94                  & 49                 & 67                 & 80                  & 73                 & 105                & 129                 & 53                 & 73                 & 86                  & 64                 & 89                 & 104                 & 68                 & 96                 & 116                 \\
MSR-GCN~\cite{Dang21}                                          & 88           & 118          & 142           & 90           & 113          & 136           & 90                 & 122                & 148                 & 103                & 134                & 155                 & 101                & 135                & 160                 & 74                 & 98                 & 121                 & 103                & 143                & 173                 & 87                 & 111                & 132                 & 84                 & 106                & 122                 & 91                 & 120                & 143                 \\
MRT~\cite{wang21}                                  & 89 & 121 & 161 & 79 & 108 & 145 & 69 & 100 & 147 & 97 & 133 & 174 & 71 & 96 & 127 & 66 & 88 & 117 & 83 & 113 & 149 & 72 & 98 & 132 & 67 & 92 & 121 & 77 & 105 & 141              \\
siMLPe~\cite{guo2022back}                                  & 95 & 125 & 141 & 82 & 114 & 134 & 63 & 93 & 115 & 124 & 174 & 212 & 61 & 80 & 92 & 50 & 67 & 79 & 83 & 116 & 138 & 59 & 81 & 90 & 72 & 99 & 116 & 77 & 106 & 124              \\ 
XIA~\cite{guo21}                                     & 82           & 116          & 142           & 69           & 97           & 120           & \textbf{52}        & 79                 & 104                 & 95                 & 137                & 171                 & 58        & 80        & 93         & 51        & 70        & \textbf{84}         & 70        & 105       & 134        & \textbf{53}        & \textbf{73}        & \textbf{88}         & 63                 & 88                 & 104                 & 66        & 94                 & \textbf{116}                 \\ 
Ours                        &       \textbf{68} & \textbf{95} & \textbf{115} & \textbf{66} & \textbf{95} & \textbf{116} & \textbf{52} & \textbf{78} & \textbf{103} & \textbf{86} & \textbf{124} & \textbf{150} & \textbf{54} & \textbf{76} & \textbf{91} & \textbf{47} & \textbf{68} & \textbf{84} & \textbf{59} & \textbf{86} & \textbf{108} & \textbf{53} & 77 & 94 & \textbf{53} & \textbf{77} & \textbf{94} & \textbf{60} & \textbf{86} & 121 \\ \hline
\end{tabular}}
\caption{Results in millimeters for ExPI Unseen actions split. On average, we outperform the baseline considered over short and long time horizons. } 
\label{tab:unseen_ame}
\end{table*}
